Automatic verification of Finite Variant Property beyond convergent equational theories

Computer-aided analysis of security protocols heavily relies on equational theories to model cryptographic primitives. Most automated verifiers for security protocols focus on equational theories that satisfy the Finite Variant Property (FVP), for which solving unification is decidable. However, they either require to prove FVP by hand or at least to provide a representation as an E-convergent rewrite system, usually E being at most the equational theory for an associative and commutative function symbol (AC). The verifier ProVerif is probably the only exception amongst these tools as it automatically proves FVP without requiring a representation, but on a small class of equational theories. In this work, we propose a novel semi-decision procedure for proving FVP, without the need for a specific representation, and for a class of theories that goes beyond the ones expressed by an E-convergent rewrite system. We implemented a prototype and successfully applied it on several theories from the literature.

==> results.tex <==
%%
%%% Section
%%

\section{Results}
\label{sec:results}

%stats de temps, du nombre de rules générés au cours de l’algol, la taille finale du système de ré-écriture et si l’algo montre que R est un système convergent

\begin{table*}[h!]
  \begin{tabular}{|c|c|r|r|r|c|}
  \hline
  % {\tiny notion} &
  \multirow{2}{*}{Acronym} & \multirow{2}{*}{Equations} &
                                                          \multicolumn{4}{c|}{Comments
                                                          and
                                                          experiments}
    \\
    \cline{3-6}
    & & time (s) & \# rules & $|\R|$ & Conv \\
  \hline
  \hline
  ACI & AC$(+)$ $\cup$ $\{ x + x = x \}$ &  $5.30$  & $54231$ & $6$
      & yes \\
  \hline
  %\hline
  ACN & AC$(+)$ $\cup$ $\{ x + x = 0 \}$ &  $35.12$ & $399143$ &
                                                                    $14$
      & yes \\
  \hline
  % {\tiny XOR} &
  $\XOR$ & AC$(+)$ $\cup$ $\{ x + 0 = x, x + x = 0\} $ & $1.60$ &
                                                                     $38468$
      & $8$ & yes \\
  \hline
  % {\tiny homomorphy} &
  h & $\{ h(x+y) = h(x) + h(y) \}$ &  \multicolumn{4}{c|}{n.a.} \\
  %   & same operator + on inputs and outputs &  & & & \\
  \hline
  % {\tiny XOR and homomorphy} &
  % $\XOR$h & $\XOR$$\cup$ h &  & & & \\
  % \hline
  % \tiny homomorphy$^{\text{in,out}}$ &
  h$(+_{\text{in}},+_{\text{out}})$  & $\{h(x +_{\text{in}} y) = h(x) +_{\text{out}}
                         h(y)  \}$ &  \multicolumn{4}{c|}{n.a.} \\
  %  & different operators on inputs and outputs &  & & & \\
  \hline
  % {\tiny XOR and homomorphy$^{\text{in,out}}$} &
  $\XOR$h$(+_{\text{in}},+_{\text{out}})$ & $\XOR$ $\cup$
                                            h$(+_{\text{in}},+_{\text{out}})$
                                                        &  $2.14$ &
                                                                       $40841$
      & $17$ & yes \\
  %  & with $+_{\text{in}}=+$, &  & &  & \\
  %  &  and $+_{\text{out}}=+$ over operands of the form $h()$ & & & & \\
    \hline
      % {\tiny Abelian Group} &
  % $\AG$$(+,0)$ & AC $\cup$ $\{ x + 0 = x, x + (-x) = 0\}$ &  & & & \\
  % \hline
  % {\tiny Abelian Group} &
  $\AG$$(*,1)$ wRc & AC$(*)$ $\cup$ $\{ x * 1 = x, x * x^{-1} = 1\}$ &
                                                                   $446.13$
                                                                   &
                                                                       $529919$
      & $52$ & yes\\
  \hline
  % {\tiny Diffie Hellman} &
  DH wRc & $\AG$$(*,1)$ $\cup$ $\{ exp(x,1) = x, $  & $1020.41$ &
                                                                  $827959$
      & $99$ & yes \\
        & $ exp(exp(x,y),z) = exp(x,y*z)\}$ &  & & & \\
    \hline
  Bilinear Pairing wRc & see example file & $3053.88$ & $1402732$ &
                                                                    $194$ & no \\ %  Bilinear\_Pairing\_with\_Rn\_conv \\
    \hline
  %  \textcolor{red}{$\AG$+} & $\AG$ with Encryption/Decryption (El Gamal) &  & & & \\
  %  \hline
    $\AG$h$(*_{\text{in}},*_{\text{out}})$ wRc &
                                                              $\AG$$(*,1)$
                                                              $\cup$
                                                              h$(*_{\text{in}},*_{\text{out}})$
                           & $1013.59$ & $815169$ & $101$ & yes \\
    \hline
    ElGamal-mixnet~\cite{usenix-mixnet} & see example file & $0.25$ & $276$ & $15$ & yes \\
    \hline
    ElGamal-mixnet-reenc~\cite{usenix-mixnet} & see example file & $0.40$ & $428$ & $19$ & yes \\
    \hline
     Toy example 1 & $g(x,y) = f(x,z)$ & $0.15$ & $218$ & $14$ & no
    \\
 &  $h(x) = 0$ &  & & & \\
                   &  $f(0,z) = p(x,z)$ &  & & & \\
    \hline
    Toy example 2 & $g(x,y) = f(x,x,z)$ &  $0.13$ & $159$ & $12$ &
                                                                      no \\
 &  $h(x,x) = 0$ &  & & & \\
 &  $f(0,x,z) = p(x,z)$ &  & & & \\
    \hline

\end{tabular}

  \caption{List of some theories that can be handled by our tool, and
    experimental results. We indicate the total number of rules
    generated, the final size of $\R$ at the end, and if the tool is
    able to prove its convergency. }
  \label{tab:theories}
\end{table*}

We developed a prototype implementing our semi-decision procedure in
OCaml and used Maude version 3.4~\cite{maude} as backend. Our source code and
examples are available in \cite{prototypeFVP}.
We successfully tested it on several theories with known FVP from the
literature (e.g. $\XOR$, $\AG$, Diffie-Hellman bilinear pairing). We also showed that many of these equational theories augmented with a homomorphic symbol with different group operators also satisfy the FVP. This is for example the case for $\XOR$, $\AG$, ElGamal and (a)symmetric encryption. Finally, we also provide several toy examples showing that the prototype also works on equational theory without AC-convergent rewrite system representation.
    
Table~\ref{tab:theories} provides information about a selection of
handled theories of different kinds, as well as experimental results
obtained on a \textcolor{red}{MacBook Pro M1}.  In this table, we
denote by AC$(+)$ (resp. AC$(*)$) the AC equational theory for the $+$
(resp. $*$) operator. The equational theory
h$(+_{\text{in}},+_{\text{out}})$ has some specificities as operators
on inputs and outputs mais be different. Nevertheless they need to
satistfy some properties: $+_{\text{in}}$ corresponds to a commutative
group operator, while $+_{\text{out}}$ needs to be a commutative group
operator over outputs of the $h$ function (but is not necessarily
commutative over other kinds of operands). Same notation is used for
the multiplicative case.
More examples can be found in
\cite{prototypeFVP}, in the \texttt{examples} folder, where each file
contains the material to run the experiment on one target equational theory,
but also already time/size/convergency results we obtained on our
laptop.






% ``weak'' homomorphic symbol, attention c'est plus général en termes
% mathématiques mais pas en termes de réécriture.



